Enhancing Mathematical Problem Solving in LLMs through Execution-Driven Reasoning Augmentation

Mathematical problem solving is a fundamental benchmark for assessing the reasoning capabilities of artificial intelligence and a gateway to applications in education, science, and engineering where reliable symbolic reasoning is essential. Although recent advances in multi-agent LLM-based systems have enhanced their mathematical reasoning capabilities, they still lack a reliably revisable representation of the reasoning process. Existing agents either operate in rigid sequential pipelines that cannot correct earlier steps or rely on heuristic self-evaluation that can fail to identify and fix errors. In addition, programmatic context can distract language models and degrade accuracy. To address these gaps, we introduce Iteratively Improved Program Construction (IIPC), a reasoning method that iteratively refines programmatic reasoning chains and combines execution feedback with the native Chain-of-thought abilities of the base LLM to maintain high-level contextual focus. IIPC surpasses competing approaches in the majority of reasoning benchmarks on multiple base LLMs. All code and implementations are released as open source.

==> sections/7_acknowledgements.tex <==
% \section{Acknowledgments}
% This material is based upon work supported by XX under Grant No. XX \footnote{The grant number is redacted for review purposes}.

==> sections/8_disclaimer.tex <==
\section{AI Usage Disclaimer}

ChatGPT was used to provide feedback on quality, assist with some grammatical refinement and articulation, and support understanding and exploration of existing mathematical concepts for framing the proposed method. However, all revisions were carefully considered and manually done. All ideas, experimental designs, analyses, and conclusions were developed by the authors, who take full responsibility for the contents of the paper. The judging agent codebase, originally written by the authors, was later enhanced with ChatGPT to improve robustness and evaluation reliability, and was reviewed and verified by the authors.
